Online and Offline Robot Programming via Augmented Reality Workspaces

Robot programming methods for industrial robots are time consuming and often require operators to have knowledge in robotics and programming. To reduce costs associated with reprogramming, various interfaces using augmented reality have recently been proposed to provide users with more intuitive means of controlling robots in real-time and programming them without having to code. However, most solutions require the operator to be close to the real robot's workspace which implies either removing it from the production line or shutting down the whole production line due to safety hazards. We propose a novel augmented reality interface providing the users with the ability to model a virtual representation of a workspace which can be saved and reused to program new tasks or adapt old ones without having to be co-located with the real robot. Similar to previous interfaces, the operators then have the ability to program robot tasks or control the robot in real-time by manipulating a virtual robot. We evaluate the intuitiveness and usability of the proposed interface with a user study where 18 participants programmed a robot manipulator for a disassembly task.

==> Makefile <==
# Makefile for building PDFs from LaTeX projects
# 2020 - Mattia Racca
#
# This makefile automatizes the compilation of complex LaTeX projects
# (e.g. a PhD thesis), with separate chapters, tikz figures and bibliography.
#
# Example of folder structure I use:
#
# thesis/
# ├── root.tex
# ├── template.sty
# ├── template.cls
# ├── chapters/
# │   ├── 01_chapter.tex
# │   └── 02_chapter.tex
# ├── figures/
# │   ├── tikz_plot.tex
# │   ├── another_tikz_plot.tex
# │   ├── cool_figure.pdf
# │   └── picture.png
# └── miscellanea/
#     ├── literature.bib
#     ├── acronyms.tex
#     └── symbols.tex
#
# Rules available:
#  all:         compiles the final .pdf with pdflatex
#  clean:       removes temporary junk files pdflatex create
#  reset_tikz:  touches all .tex of tikz illustrations (so that they need to be recompiled)
#  info:		prints tracked files

# Variable definitions

TARGETS = root.pdf
CHAPTER_FOLDER = chapters
BIBFILE_FOLDER = miscellanea
TIKZ_FOLDER = figures
SUPPORT_FOLDER = miscellanea

CHAPTERS := $(wildcard $(CHAPTER_FOLDER)/*.tex)
BIBFILES := $(wildcard $(BIBFILE_FOLDER)/*.bib)
TIKZS := $(wildcard $(TIKZ_FOLDER)/*.tex)
SUPPORTS := $(wildcard $(SUPPORT_FOLDER)/*.tex)

JUNK = junk.aux junk.auxlock junk.bbl junk.blg junk.dvi junk.log \
junk.out junk.acn junk.acr junk.alg junk.asc junk.asp junk.ist junk.toc junk.ase

# Rules

all: $(TARGETS)

$(TARGETS): $(CHAPTERS)
$(TARGETS): $(TIKZS)
$(TARGETS): $(SUPPORTS)
$(TARGETS): %.pdf: %.bbl
$(TARGETS): %.pdf: %.tex
	pdflatex -shell-escape $<
	pdflatex -shell-escape $<

$(TARGETS:.pdf=.bbl): $(BIBFILES)
$(TARGETS:.pdf=.bbl): %.bbl: %.tex
	pdflatex -shell-escape $<
	# makeglossaries $*
	# bibtex $*

clean:
	rm -f $(subst junk,$(TARGETS:.pdf=),$(JUNK))
	rm -f $(CHAPTERS:.tex=.aux)
	rm -f $(TIKZS:.tex=.log)
	rm -f $(TIKZS:.tex=.aux)
	rm -f $(SUPPORTS:.tex=.aux)

reset_tikz:
	touch $(TIKZS)

info:
	# Project Summary for $(TARGETS):
	#
	# chapters:
	# $(subst $(CHAPTER_FOLDER)/,,$(CHAPTERS))
	#
	# bib files:
	# $(subst $(BIBFILE_FOLDER)/,,$(BIBFILES))
	#
	# support files:
	# $(subst $(SUPPORT_FOLDER)/,,$(SUPPORTS))
	#
	# tikz figures:
	# $(subst $(TIKZ_FOLDER)/,,$(TIKZS))

